Local Certification of Graphs with Bounded Genus

Naor, Parter, and Yogev [SODA 2020] recently designed a compiler for automatically translating standard centralized interactive protocols to distributed interactive protocols, as introduced by Kol, Oshman, and Saxena [PODC 2018]. In particular, by using this compiler, every linear-time algorithm for deciding the membership to some fixed graph class can be translated into a $\mathsf{dMAM}(O(\log n))$ protocol for this class, that is, a distributed interactive protocol with $O(\log n)$-bit proof size in $n$-node graphs, and three interactions between the (centralizer) computationally-unbounded but non-trustable prover Merlin, and the (decentralized) randomized computationally-limited verifier Arthur. As a corollary, there is a $\mathsf{dMAM}(O(\log n))$ protocol for the class of planar graphs, as well as for the class of graphs with bounded genus. We show that there exists a distributed interactive protocol for the class of graphs with bounded genus performing just a single interaction, from the prover to the verifier, yet preserving proof size of $O(\log n)$ bits. This result also holds for the class of graphs with bounded demi-genus, that is, graphs that can be embedded on a non-orientable surface of bounded genus. The interactive protocols described in this paper are actually proof-labeling schemes, i.e., a subclass of interactive protocols, previously introduced by Korman, Kutten, and Peleg [PODC 2005]. In particular, these schemes do not require any randomization from the verifier, and the proofs may often be computed a priori, at low cost, by the nodes themselves. Our results thus extend the recent proof-labeling scheme for planar graphs by Feuilloley et al. [PODC 2020], to graphs of bounded genus, and to graphs of bounded demigenus.

==> s1-outline.tex <==
% !TEX root = main-PLS-surface.tex

\section{Old material where to pick useful stuff}

In this paper we present a proof-labeling scheme for the property of being embeddable in a given topological surface. 
It is known that surfaces are characterized by the orientability (being orientable or not) and the genus, which is an integer. Thus we design a family of schemes, one for each surface. 
For orientable surface, the genus is intuitively the number of holes in it: the sphere is the orientable surface of genus 0, the torus is the orientable surface of genus 1 etc.   

\paragraph{A constructive characterization of the surfaces}

Let us start by showing how surfaces are characterized, before going to graphs.

The nature of a surface (orientability and genus) is defined through cutting operations (like one could do with scissors) or, in a dual way, through gluing operations.
%Basically if one makes enough cuts in the surface, one ends up with a "flat surface", and then if one reglues the borders, one can rebuild the surface.
%The structure of the cuts, or dually which border has to be glued with other, completely characterizes the surface. 

Let us start with an example, the torus, that is the orientable surface of genus 1.
In Figure~\ref{fig:cutting-loops}, the torus is represented with two \emph{loops}: a green one and a red one that meet in one point, that is called the \emph{basepoint}. If we cut along these loops, and unfold the surface on the plane, we get the rectangle on the right, with the information about the origin of the border. This rectangle is called a \emph{polygonal scheme}. In general a polygonal scheme is a polygon whose side are labeled (here the labels are the colors) and oriented.

Now, conversely, if we take the rectangle and glue  the red paths together and the green paths together, then we rebuild the torus.
A subtlety is the orientation of these paths: to get the torus one has to glue the paths with the arrows in the consistent orientation (the head of the arrows together and the back of the arrows together). Without entering too much into details now, gluing in another way would create another surface (of genus 0 or non-orientable). 
In general given a polygonal scheme, one can recreate the surface by identifying the side with equal labels, taking care of having consistent orientations.

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.25]{figures/fig-torus-cut.png}
&
\includegraphics[scale=0.4]{figures/fig-torus-flat-map.png}
\end{tabular}
\caption{\label{fig:cutting-loops} Cuts for the torus.}
\end{center}
\end{figure} 

A more complicated example of the gluing process is detailed in Figure~\ref{fig:double-torus} for the double torus (the orientable surface of genus 2), where the polygonal scheme is an octagon. 

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.35]{figures/2-torus-1.png}
&
\includegraphics[scale=0.35]{figures/2-torus-2.png}
\\
Polygonal scheme for the double torus.
&
Merging the red paths.
\\
\includegraphics[scale=0.35]{figures/2-torus-3.png}
&
\includegraphics[scale=0.35]{figures/2-torus-4.png}
\\
Merging the yellow paths.
&
Identifying two copies of the basepoint. 
\\
\includegraphics[scale=0.35]{figures/2-torus-5.png}
&
\includegraphics[scale=0.35]{figures/2-torus-6.png}
\\
Identifying the green loops by creating a 1st handle.
&
Identifying the green loops by creating a 2nd handle.
\end{tabular}
\includegraphics[scale=0.35]{figures/2-torus-7.png}
\\
Changing the aspect to make it look nice.
\caption{\label{fig:double-torus} The gluing process of the double torus.}
\end{center}
\end{figure}

The key point here is that all there is to know about the torus is given by the rectangle on the right, saying what to glue and with which orientation. 
This is actually a general statement, indeed the \emph{classification of the surfaces} (see Theorems~\ref{th:classification-orientable} and \ref{th:classification-non-orientable} later) states that:
\begin{itemize}
\item all the polygonal schemes define surfaces
\item all topological surface have a set of loops (called a \emph{loop system}) such that cutting along these loops, provides a canonical polygonal scheme associated with this surface.
\end{itemize}  

For example the canonical polygonal scheme for the torus is the one given in Figure~\ref{fig:cutting-loops}, but other polygonal schemes when glued also give the torus.
  
\paragraph{Embedded graph}

We now introduce graphs on surfaces.
A graph embedded in a torus is represented in Figure~\ref{fig:graph-on-torus}, on the left. Here ``embedded in a surface'' means that the graph is drawn on the surface and that there is no crossings of edges. For example a planar graph is a graph that can be embedded on a sphere (or equivalently on the plane).
Now if we apply the cutting operation described above, we get a picture like the one on the right in Figure~\ref{fig:graph-on-torus}. Note that some edges are cut into two half-edges. 
Now by gluing the green paths together and the red paths together we can rebuild the original surface and also the graph embedded on it (by regluing the half-edges together).

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.3]{figures/fig-graph-on-torus.png}
&
\includegraphics[scale=0.4]{figures/fig-flat-map.png}
\end{tabular}
\caption{\label{fig:graph-on-torus} Graph embedded on the torus.}
\end{center}
\end{figure} 

\paragraph{First attempt for certification: planarity and polygons.}

Given a picture like the one on the right of Figure~\ref{fig:graph-on-torus}, a strategy comes to mind to certify that the graph is embeddable on some surface $X$. 
One just has to ask the prover to:
\begin{enumerate}
\setlength{\itemsep}{1pt}
\item find a loop system of the surface  
\item \label{item:edge-cut} describe and certify how the edges of the graph are cut by these loops
\item certify the planarity of the graph with the half edges
\item certify that the polygonal scheme is the one of surface $X$.
\end{enumerate}

A problem here is Item~\ref{item:edge-cut}. Indeed, 
to be used algorithmically the loops have to be defined in a combinatorial way. This can be done in the centralized setting, by having the loops going alternating between faces and nodes. But in our distributed setting, it is not clear how one could certify that consistency of these loops without using very large certificates. Therefore we are forced to use loops that follow the edges, that is that are cycles of the graph. Unfortunately this is not always possible. Consider Figure~\ref{fig:K33-torus-paths} where a $K_{3,3}$ is drawn on the torus. For this graph, it is not possible to find two cycles forming a loop system: any couple of cycles that would cut the torus would share an edge, and the theory of surfaces only takes care of loop system where the only point in common is the basepoint.  
Note that $K_{3,3}$ is neither a degenerate case nor an exception: any graph embedded in the torus with maximum degree at most 3 would be in the same situation as no node can be the basepoint.

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.3]{figures/fig-K33-torus.png}
\end{tabular}
\caption{\label{fig:K33-torus-paths} $K_{3,3}$ on the torus.}
\end{center}
\end{figure}

\paragraph{New tools are required}

The issue described above (not being able to have disjoint cycles as loops) is not often considered in the literature. Basically, in distributed literature, bounded genus is not very present and authors present algorithms that do not need this structural decomposition, and in the centralized literature, the problem is not that critical.
Indeed, in the centralized case, either one can use loops that do not follow the edges, or can modify the graph a bit to avoid the problem. For example one can add a few nodes inside each face to create more paths, and increase the degree of the vertices, without harming the embeddability properties while only increasing the number of nodes by a small factor. This way one can directly use the classification theorem. In the distributed setting it is not so clear how to define, describe and certify efficiently such a transformation. 

In a nutshell, in our context it is not possible to apply the known tools, e.g. the classification theorem. Instead we define an alternative decomposition of the surfaces. To be sure that this decomposition is well-defined, we have to go back to some topological notions, that are usually unnecessary, when one can use the classification theorem.

\paragraph{Second attempt: duplication and Euler formula.}

At first sight, our approach is similar to the one first attempt. We ask the prover to:
\begin{enumerate}
\item perform some specific operations on the graph that reduce the genus until the graph is planar
\item describe the modified graph to the nodes and certify it is planar. 
\item describe how to undo the operations, to recover the original graph and certify the correctness of these operations. 
\end{enumerate}

The specific operation to decrease the genus is what we call a \emph{cycle duplication}. It simply consists in cutting along some specific cycle as in Figure~\ref{fig:duplication}, duplicating the nodes of it, and adding two faces to patch the holes we have created. Not every cycle can be used for this operation: the operation should not disconnect the graph. Intuitively, in the orientable case, this means that the cycle should cut a handle.

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.5]{figures/fig-cycle-duplication-1.png}
&
\includegraphics[scale=0.5]{figures/fig-cycle-duplication-2.png}
\end{tabular}
\vspace{-1.5cm}

\includegraphics[scale=0.55]{figures/fig-cycle-duplication-3.png}
\end{center}
\caption{\label{fig:duplication} Illustration of the cycle duplication. Here we cut along the cycle $(v_1, v_2, v_3)$. That is we duplicated these nodes: now they are green, and have two version: $v_i^a$ and $v_i^b$. The "interior" of the surface is in pink. Now we add two yellow faces to patch the holes. This makes the handle disappear: this part of the graph is now "flat". Note that on the yellow face on the left, reading the nodes in the order $1,2,3$ makes us go counter-clock wise, whereas for the face on the right we go clockwise.}
\end{figure}

This operation decreases the genus. We can check that using Euler formula\ioanmp{La formule ne marche que pour les graphes connexes. Il me semble que beaucoup de choses requi\`erent la connexit\'e du graphe en entr\'ee (y compris le 2-cell embedding), on devrait l'affirmer depuis le d\'ebut pour ne plus avoir \`a en parler.}. 
Remember that Euler formula is the following relation between the number of vertices $|V|$, the number of edges $|E|$, the number of faces $|F|$ and the genus $k$:

$$ \vert V \vert -  \vert E \vert  +  \vert F  \vert =  2 - 2k \text{ (orientable case) or } 2-k \text{ (non-orientable case).} $$

Now the operation creates the same number of vertices and edges, and creates two new faces, thus thanks to the formula, we know that the genus is strictly smaller.
Hence after performing this operation some number of times, we get a planar graph, as planned.

We ask the prover to describe how the vertices of the duplicated cycles are split (we call this the \emph{splitting}), and then to certify that the graph with the split nodes is planar. For the planarity we use the scheme from the literature \cite{FeuilloleyFRRMT}. 

\paragraph{Verification and orientation} 

Now there are two main things that the nodes have to check:
\begin{enumerate}
\item The splitting of the nodes announced by the prover is correct.
\item The operations of the prover do lead to the surface $X$.
\end{enumerate} 

As we will see the verification of the splitting requires some care, but is doable. 
One of the obstacle being the fact that we somehow need to describe for each split node which neighbor is adjacent to which copy, without exploding the certificate size even if the degree is large. 
This is done using the fact that the degeneracy of the graph is bounded (a technique already introduced in \cite{FeuilloleyFRRMT}, that we generalize).

The key challenge is to keep track of the orientation. To exemplify why this is problematic, consider a simple case: the certification that the graph is embeddable in the torus. For this, the prover only perform one cycle duplication, and then certify that the graph is planar. Now consider the two faces that have been created by the duplication (the yellow faces in Figure~\ref{fig:duplication}), and orient them in such a way that the copies of the nodes are visited in the same order (\emph{e.g.} $(v_1^a, v_2^a, ...)$ and $(v_1^b, v_2^b,...)$). If these orientations are in opposite (one clockwise and one anti-clockwise) then the gluing is correct and we recover a torus, but if they are identical, the surface obtained by gluing is not a torus, it is the non-orientable surface of genus 1: the Klein bottle. Therefore it is crucial to allow the nodes to detect such orientation problems.

\paragraph{Solving the orientation problem} 

The way we handle the orientation problem is by asking the prover to perform more operations on the graph. Specifically, we ask the prover to perform more duplications (on paths this time), in order to have all split nodes on the border of a \emph{unique face}. The key point here is that given an orientation of this face, the nodes can undo the path duplications, and keep track of the orientation. 

The path duplication consists in iteratively taking two of the faces that have split nodes, finding a path between them, and duplicating the path, as in Figure~\ref{fig:path-duplication}.

\begin{figure}[!h]
\begin{center}
\begin{tabular}{c}
\includegraphics[scale=0.5]{figures/fig-path-duplication-1.png}\\
\includegraphics[scale=0.5]{figures/fig-path-duplication-2.png}
\end{tabular}
\caption{\label{fig:path-duplication} Path duplication. Two faces created by cycle duplication (possibly with other path duplications) are merged into one by duplicating a path. The number of yellow faces is reduced by one. Note that the green names for the vertices at the beginning should be of the form $v_i^a$ etc.}
\end{center}
\end{figure} 

To certify the existence of the unique special face at the end of the procedure, we use the fact that the scheme of \cite{FeuilloleyFRRMT} certifies, as a by-product, which nodes are on the outerface of the planar drawing. 

\paragraph{Lower bound on genus}

In order to certify that a graph is of genus $k$, we show that it cannot be embedded in a surface of genus $k-1$, and that it can be embedded in a surface of genus $k$. The negative side goes by reasoning about minors. As graphs of a bounded genus form a class that is closed by minors, there exists a characterization by a finite family of forbidden minors, thanks to the celebrated results of Robertson and Seymour. It is folklore that a graph has a specific minor can be certified locally with $O(\log n)$ bits (see eg \cite{FeuilloleyFRRMT}), thus one can certify that a graph cannot be embedded on a surface of some given genus with $O(\log n)$ bits certificates. 


\ivan{I think that the Outline is very nice and original (the way it is written, the approach).
But it is suddenly cut. why? We want to continue the reading!!
There is already enough material in the document to continue the narrative.
Maybe the Outline section should continue developing the case of the torus.
The subsection "More duplications and the use of outerface” could be replaced
by figure 6, 7, 8 and 9  (all of them related to the torus!!!)  2-cell embeddings, duplications of paths,
putting all the duplicated vertices in the outerface,etc. 
In Section 3 I would discuss the certificates for the torus.
In Section 4 I would explain the general case (easier to read once the torus is understood, but full of subtilities)}




==> s2-preliminary-surfaces_-_old.tex <==
% !TEX root = main-PLS-surface.tex

\newpage 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Definitions, and Formal Statement of the Problem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section contains a brief introduction to graphs embedded on surfaces, and provides the formal statement of our problem. Most of the notions mentioned in this section are standard, and we refer to, e.g.,  Massey et al.~\cite{massey1991basic} for more details. 

%--------------------------------------------------------------------------------------------------------
\subsection{Closed Surfaces}
%--------------------------------------------------------------------------------------------------------

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Construction} 
\label{sec:surface} 
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

So-called \emph{closed surfaces} can merely be obtained by the following construction, where $D$  is a closed unit disk in~$\R^2$. First, divide the boundary of~$D$ into $2 k$ arcs, for some $k\geq 1$, and provide each arc with a direction (clockwise or counterclockwise). Next, provide a color to each arc, in such a way that every color is attributed to exactly two arcs. Finally, for every pair of arcs with the same color,  identify the two arcs by glueing them together  while respecting their directions. See Figure~\ref{fig:torus-construction}. 

\begin{figure}[htb]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.2]{figures/fig-torus-cut.png}
&
\includegraphics[scale=0.3]{figures/fig-torus-flat-map.png}
\end{tabular}
\caption{Construction of a closed surface}
\label{fig:torus-construction} 
\end{center}
\end{figure} 


For instance, if the boundary of~$D$ is divided in two arcs with opposite direction, then the surface resulting from this construction is  the sphere, denoted by~$S^2$, or~$\T_0$. Instead, if the two arcs are provided with the same direction, then the resulting surface is  the  projective plane. If the boundary of~$D$ is divided in four arcs, where any two opposite arcs are provided with an identical color but a different direction, then the resulting surface is the  torus, denoted by~$\T_1$. Instead, if two opposite arcs are given the same direction, while the other two are given different directions, then the resulting surface is the Klein bottle. Note that the Mobius strip is not a closed surface, as it has a boundary. 

A \emph{characteristic word} associated to a surface constructed as above is a word with $2k$ letters obtained by traveling along  the boundary of~$D$ clockwise, and by writing the successive colors of the arcs, either~$a$ for an arc colored~$a$ with clockwise direction, or~$a^{-1}$ for an arc colored~$a$ with counterclockwise direction. In particular,  $aa^{-1}$, $aa$, $aba^{-1}b^{-1}$, and $aba^{-1}b$ are the respective characteristic words of the sphere, the projective plane, the torus, and the Klein bottle. 

The surfaces resulting from this construction can be orientable (e.g., a torus) or not (e.g., a Klein bottle), depending on the directions given to the pairs of arcs that are identified. For defining the orientation of surfaces, and their genus, as well as for the sake of conveniency when manipulating surfaces, it is convenient to introduce some basic notions of topology, as done hereafter. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Orientability} 
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

Recall that a \emph{topological space} is a pair $(X, T)$ where $X$ is a set, and $T$ be a topology on $X$ (e.g.,  $T$ is a collection of subsets of $X$,  whose elements are called open sets). A topological space may merely be denoted by $X$ if there is no ambiguity about the topology on~$X$. Also recall that a function $f:X\to Y$ is \emph{continuous} if the inverse image of every open set of $Y$ is open in~$X$. A \emph{homeomorphism} is a bijection that is continuous, and whose inverse is also continuous. Two homeomorphic topological spaces are said to be \emph{equivalent}. A topological space is \emph{disconnected} if it is the union of two disjoint non-empty open sets, and is \emph{connected} otherwise. A subset of a topological space is said to be connected if it is connected under the induced subspace topology, and the connected subsets that are maximal by inclusion are the \emph{connected components}. 

A closed surface can be alternatively defined as a connected compact Hausdorff space\footnote{Two elements $x,y\in X$ can be separated if there exists a neighborhood $N_x$ of~$x$, and a neighborhood $N_y$ of~$y$ such that $N_x\cap N_y=\varnothing$. $X$~is a Hausdorff space if all distinct points in~$X$ are pairwise separable. } that is locally homeomorphic to a disk of~$\R^2$. For defining orientability of the closed surface~$X$, we use the notion of  \emph{curve}, defined as a  continuous  function $C:S_1 \to X$, where $S_1$ denotes the unidimensional sphere (homeomorphic to, e.g., the trigonometric circle). A curve is \emph{simple} if it is injective.  A simple curve~$C$ is \emph{orientable} if one can define the left side and the right side of the curve at every point of the curve in a consistent manner.  Specifically, a curve~$C$ is orientable if, for every $x \in C$, there exists a neighborhood $N_x$ of $x$ such that $N_x \smallsetminus C$ has two connected components, one called the left side $L(N_x)$ of $N_x$, and the other the right side $R(N_x)$ of $N_x$, such that, for every $x,x' \in C$ and every $y\in X$, 
\[
(y \in N_x \cap N_{x'})    \land   (y \in L(N_x)) \; \Longrightarrow \; y \in L(N_{x'}).
\]
A closed surface $X$ is orientable if every simple curve of  $X$ is orientable. It is easy to check that orientability is a topological invariant. That is, if  $X$ and $Y$ are two homeomorphic topological spaces,  then $X$ is orientable if and only if $Y$ is orientable. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Genus of a Surface} 
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

An orientable closed  surface surface $X$ is of \emph{genus}~$0$ if it is homeomorphic to a closed surface constructed as in Section~\ref{sec:surface} with characteristic word $aa^{-1}$ (i.e.,  if it is homeomorphic to a sphere), and, for $k \geq 1$, $X$~is of \emph{genus}~$k$ if it is homeomorphic to a surface with characteristic word 
$$(a_1b_1a_1^{-1}b_1^{-1})(a_2b_2a_2^{-1}b_2^{-1}) \dots (a_kb_ka_k^{-1}b_k^{-1}).$$ 
The classification theorem of  orientable closed surfaces (see, e.g., \cite{Brah22}) states that every orientable closed surface has a genus. That is, for every orientable surface~$X$, there exists a unique~$k\geq 0$ such that $X$ is of genus~$k$. 
 
It follows from the classification theorem that,  for every orientable closed surface~$X$ of genus~$k$, and for every $x \in X$,  there exists  $2k$ simple curves $C_1,  \dots, C_{2k}$ such that the intersection of any two of these curves  is reduced to the singleton~$x$.  Moreover, $X\smallsetminus \cup_{i=1}^{2k}C_i$ is homeomorphic to a disk whose  boundary is divided into $2k$ directed  and colored arcs. In the following, we refer to $X\smallsetminus \cup_{i=1}^{2k}C_i$ as the surface resulting from ``cutting $X$  along the cycles $C_1, \dots, C_{2k}$''. The cycles $C_1, \dots, C_{2k}$ form a \emph{collection of cut curves} of $X$. 

Since every pair of orientable closed  surfaces of genus~$k$  are homeomorphic, a unique notation can be adopted for these surfaces. An orientable closed  surface of genus~$k$ is denoted by~$\T_k$. 

\medskip

Interestingly, the genus can also be defined for non-orientable closed surfaces. For $k\geq 1$, a non-orientable closed surface surface is said of \emph{genus}~$k$ if it is homeomorphic to a a closed surface constructed as in Section~\ref{sec:surface} with characteristic word 
$$a_1a_1\, a_2a_2 \, \dots \, a_ka_k. $$ 
As for orientable surfaces, the classification theorem of  non-orientable closed surfaces (see, e.g., \cite{Brah22}) states that every non-orientable closed surface has a genus. That is, for every  non-orientable closed surface~$X$, there exists a unique~$k\geq 0$ such that $X$ is of genus~$k$.  Again, every pair of non-orientable closed  surfaces of genus~$k$  are homeomorphic. A non-orientable closed  surface of genus $k$ is denoted by~$\NT_k$. 

\paragraph{Remark.} The following provides a characterization of surfaces that can also serve as an alternative definition for orientable and non-orientable closed surfaces of a given genus. 
\begin{itemize}
\item An orientable closed surface of genus~$k\geq 0$ consists of a sphere to which $k$ handles are attached, where a handle is obtained by deleting the interior of two disjoint disks on the surface of the sphere, orienting clockwise the boundary of one cycle, orienting counterclockwise the boundary of the other  cycle, and gluing the two cycles in respecting their orientation. 
\item A non-orientable closed surface of genus~$k\geq 1$ consists of a sphere in which the interior of $k$~disjoint disks on the surface of the sphere are deleted, and each resulting hole is closed by identifying pairs of diametrically opposite points on its boundary. 
\end{itemize}


%--------------------------------------------------------------------------------------------------------
\subsection{Graphs Embedded on Surface} 
%--------------------------------------------------------------------------------------------------------

In this section, we recall standard notions related to graph embeddings on surfaces, and we refer to Mohar and Thomassen  \cite{mohar2001graphs} for more details. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Topological Embedding}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

Given a graph $ G = (V, E) $, and a topological space $( X, T)$,  a \emph{topological embedding } of  $G$ on $(X, T)$ is given by (1)~an injective  mapping $ f : V \rightarrow X$, and, (2)~for every edge  $e  \in E$, a continuous mapping $f_e : [0, 1] \rightarrow X$, such that
\begin{itemize}
\item for every edge $e = \{v, v'\}  \in E$,  $f_e(\{0, 1\}) =   \{f(v), f(v') \}$, and 
\item for every pair $\{e, e'\}$ of distinct edges,   $f_e(]0, 1[) \cap f _{e'}(]0, 1[)  = \varnothing$.    
\end{itemize}
In the definition of topological embedding, the latter condition is ofter referred to as the \emph{non-crossing} condition.  See Figure  \ref{fig:2cell} for two embeddings of the complete graph~$K_4$ in~$\T_1$. 

In the following, we may confuse a vertex~$v$ with its representation~$f(v)$, and an edge $e$  with its representation $f_e$ (i.e., the image $f_e([0,1])$ of $[0,1]$ by $f_e$), even referred to as~$f(e)$. The set $ \cup_{e \in E} f(e) $ is called the \emph{skeleton} of the embedding, and is denoted by~$\Sk(G)$.  Each connected component of $X \smallsetminus  \Sk(G)$ is an open set of $X$ (as complement of a close set), called a \emph{face} of the embedding. In fact, in this paper, we will abuse notation, and often refer to~$G$ instead of~$\Sk(G)$. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{2-cell embedding}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

We now recall a slightly more sophisticated, but significantly richer form of topological embedding. A \emph{2-cell embedding} is a topological embedding such that every face is homeomorphic to an open disk of~$\R^2$. 

In a 2-cell embedding, the border of a  face can  be described by giving a so-called \emph{boundary (closed) walk}, that is, an ordered list $(v_0, \dots, v_k)$ of non-necessarily distinct vertices of the graph~$G$, with $v_k =v_0$.  The vertices and   edges of a face are the images by the embedding of the vertices and edges of the boundary walk.  The  boundary  walk is however not necessarily a simple cycle, as  an edge may appear twice in the walk, once for each direction, and a  vertex may even appear many times. 

\begin{figure}
    \centering
\begin{tabular}{cc}
\includegraphics[scale=0.2]{figures/fig-K4-1}
&
\includegraphics[scale=0.2]{figures/fig-K4-2}
\end{tabular}

    \caption{Two embeddings of  $K_4$ in the torus $\T_1$. }
    \label{fig:2cell}
 \end{figure}
 
\paragraph{Example.} 

 Figure~\ref{fig:2cell} displays two embeddings of the complete graph $K_4$ in the torus~$\T_1$. The embedding on the left is not a 2-cell embedding. Indeed, this embedding results in three faces, including the two faces with boundary walk $(a,b,c,a)$ and $(a,b,d,a)$. The third face is however not homeomorphic to an open disk (there is a hole in it, resulting from the hole in the torus).  On the other hand, the embedding on the right in Figure  \ref{fig:2cell} is a 2-cell embedding. Indeed, there are two faces, including the face with boundary walk $(a,b,c,a)$. The other face is also homeomorphic to an open disk. A boundary walk of this latter face is $(d, a, b, d, c, a, d,  b, c, d)$. This can be seen by starting from $d$, traversing the edge $\{d,a\}$, and adopting the ``left-hand rule'' when entering a vertex, leading from $a$ to $b$, then back to $d$, next to~$c$, etc.  Notice that this  boundary walk uses some edges twice. It follows that the closure of a face is not necessarily homeomorphic to a closed disk, even in a 2-cell embedding.  

We complete the section by two observations. The first one will allow us to restrict attention to cycles in graphs instead of arbitrary curves in topological spaces. It also illustrates the interest of 2-cell embedding (the result does not necessarily hold for an arbitrary embeddings, as illustrated by the embedding on the left of Figure~\ref{fig:2cell}).

\begin{lemma} 
For every graph $G$, and every topological space~$X$, any 2-cell embedding  of $G$ to $X$ satisfies that 
every closed curve in $X$ is either contractible, or homotopic to a closed cycle of~$\Sk(G)$. 
\end{lemma}
% \eric{ In particular, for  $X$ to be  orientable, it suffices each closed cycle of $G$ to be  orientable }
 
The rough reason why the result holds is that, in a 2-cell embedding, any sub-path of a path traversing a face can be replaced by a sub-path following the border of the face. (This is not necessarily true for a general embedding). The second observation will allow us to use connectivity and compactness arguments. 

\begin{lemma} \label{connect}
For every graph $G$, and every topological space~$X$, if there exists a 2-cell embedding  of $G$ to $X$ then (1)~$X$ is compact, and (2)~$X$ is path-connected if and only if $G$ is connected. 
\end{lemma}

Briefly, the fact that $X$ is compact follows from the fact that, if there exists a 2-cell embedding  of $G$ to $X$, then the closure of every face is compact, and thus $X$ is compact as finite union of compact sets. Regarding the second claim, if $X$ is connected, then, for every two vertices $u,v$ of $G$, there exists a path in $X$ from $u$ to $v$, and this path is homotopic to a path in~$\Sk(G)$. Conversely, if $G$ is connected, then a path between any two element $x,y$ of $X$ can be obtained by going from $x$ to the border of the face containing~$x$, then going along the edges of $G$ to border of the face containing~$y$, and finally reaching~$y$. 
 
% Eric : morceau  garder , cela peut peut tre servir 
%  \subsubsection{Local and global orientation}
%  \eric{ ici, il faut parler orientation, j'ajoute le paragraphe suivant}
%
%Take   a  2-cell embedding of a graph $G = (V, E)$ and $v \in V$. A \emph{local rotation} in $v$ is a cyclic permutation $\pi_v$ of edges  incident in $v$, such that 
% when $ \pi_v( \{v, w\}) = \pi_v( \{v, w' \})$,  there exists a face $f$  such that $(w, v, w')$ is a factor of a boundary walk of $f$. 
% % For each $v$ of degree at least 3, there exists two local rotations,   while for each $v$ of degree at most 2  \in V \setminus V_{3^+} $, there exists a unique  local rotation. 
% 
%A  \emph{rotation system} is a sequence $(\pi_v)_{v \in V}$  when for each edge $\{v, w\} \in E$, vertices $x$ and $y$, defined by the equalities  $ \pi_v( \{v, w \}) = \{v, x \}$  and  $\pi_w( \{w, y\}) = \{w, v\}$ are such that there exists a face $f$ such that $(x, v, w, y)$ is a factor of a boundary walk of $f$. 
% 
% \begin{lemma} \cite{Yo63}
%For  any 2-cell embedding of a graph $G = (V, E)$, with no vertex of degree 2,   on a closed surface $X$, there exists a rotation system  if and only if $X$ is orientable. 
%\end{lemma}
%
%Notice that the fact that vertices of degree 2 are not relevant for embeddings, thus the restriction given by the absence of vertices of degree is not really important. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Genus  of a graph}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

For any graph $G$, if $G$ can be embedded on $\T_k$, then $G$ can be embedded on $\T_{k'}$ for every $k' \geq k$. The \emph{genus} of a graph $G$ is the smallest $k$ such that there exists an embedding of $G$ on $\T_k$. Similarly, the \emph{non-orientable} genus,  a.k.a.~\emph{demigenus}, or \emph{Euler genus} is defined as the smallest~$k$ such that there exists an embedding of $G$ on $\NT_k$. The embeddings of graphs of genus~$k$ on~$\T_k$  have a remarkable property (see, e.g.,~\cite{Yo63}).

\begin{lemma} 
Every embedding of a graph  $G$ of genus $k$  on $\T_k$ is a 2-cell embedding. 
\end{lemma}

The next result  is extremely helpful for computing the genus of a graph, and is often referred to as the Euler-Poincar\'e formula~\cite{poincare}. 

\begin{lemma}
\label{euler}
Let $G = (V, E)$, and let $X$ be a closed surface of genus~$k$. Let us consider any 2-cell embedding of $G$ to $X$,  and let $F$ be the set of faces of this embedding. If $X$ is orientable then $ \vert V \vert -  \vert E \vert  +  \vert F  \vert =  2 - 2k$. If $X$ is non orientable then $ \vert V \vert -  \vert E \vert  +  \vert F  \vert =  2 - k$.
\end{lemma}

Lemma~\ref{euler} enables to relate the genus of a graph with its \emph{degeneracy}~$d\geq 0$. Recall that, a graph $G$ is $d$-degenerate if every subgraph of $G$ has a node of degree at most~$d$.

\begin{lemma}\label{genus-implies-degeneracy}
For every $k\geq 0$, there exists $d\geq 0$ such that every graph of genus at most $k$ is $d$-degenerate. Similarly, For every $k\geq 1$, there exists $d\geq 0$ such that every graph of demigenus at most $k$ is $d$-degenerate.
\end{lemma}

\begin{proof}
\pierremp{On ajoute une ref et on enl\`eve la preuve? }
To establish the lemma, we show that, for every $c \in\Z$, there exists $d \geq 0$ such that, for every graph~$G=(E,V)$, and for every 2-cell embedding of $G$ on a closed surface~$X$, if  $|V|-|E|+|F|=c$ then there exists a vertex of $G$ with degree at most~$d$. (This suffices for establishing the lemma because being of genus at most~$k$ is closed under vertex-deletion). Let $F$ be the set of faces of the embedding. For every face $\phi\in F$, let $\deg(\phi)$ denotes the number of edges incident to~$\phi$ in the dual graph of~$G$. In other words, $\deg(\phi)$ is the length  of the boundary walk of~$\phi$. On the one hand, 
$
2 \vert E \vert  = \sum_{ v \in V} \deg(v)  =  \sum_{ \phi \in F} \deg(\phi).
$
On the other hand,  for every $\phi \in F$, $\deg(\phi) \geq 3$. It follows that 
$
2 \vert E \vert   = \sum_{ \phi \in F} \deg(\phi) \geq 3 \vert F  \vert. 
$
Therefore, $ \vert V \vert -  \vert E \vert  +  \vert F  \vert = c$ implies that 
$\vert V \vert    - \frac13  \vert E \vert \geq  c$, i.e., $\vert V \vert    - \frac16 \sum_{ v \in V} \deg(v)\geq  c$. The latter inequality can be rewritten as
$ \frac1{|V|} \sum_{ v \in V} \deg(v) \leq 6 -\frac1{|V|} 6c \leq \max \{   6,    6-6c\}. $
Since the average degree is upper bounded by $\max \{   6,    6-6c\}$, there exists a node with degree at most $\max \{   6,    6-6c\}$.
\end{proof}

%--------------------------------------------------------------------------------------------------------
\subsection{Formal Statement of the Problem}
%--------------------------------------------------------------------------------------------------------

Proof-Labeling Schemes (PLS) are distributed mechanisms for verifying graph properties. More precisely, let $\G$ be a graph family. A PLS for $\G$ is defined as a prover-verifier pair $(\mathbf{p},\mathbf{v})$, bounded to satisfy the following. Given any $n$-node graph $G=(V,E)$ whose vertices are labeled by distinct identifiers in $\{1,\dots,n\}$, the prover~$\mathbf{p}$ in a non-trustable oracle that provides every vertex $v\in V$ with a \emph{certificate}~$c(v)$. The verifier~$\mathbf{v}$ is a simple distributed protocol performed in parallel at all vertices as follows. Every vertex collects the certificates of all its neighbors, and must output ``accept'' of ``reject'', on the basis of its identifier, its certificate, and the certificates of its neighbors. The pair $(\mathbf{p},\mathbf{v})$ is a correct PLS for~$\G$ if the following two conditions hold. 


\begin{description}
\item[Completeness:] For every $G\in\G$, and for every identity-assignment to the vertices of~$G$, the (non-trustable) prover~$\mathbf{p}$ can assign certificates to the vertices such that the verifier~$\mathbf{v}$ \emph{accepts} at all nodes;
\item[Soundness:] For every $G\notin\cal{G}$, for every identity-assignment to the vertices of~$G$, and for every certificate assignment to the nodes by the non-trustable prover~$\mathbf{p}$, the verifier~$\mathbf{v}$  \emph{rejects} in at least one node. 
\end{description}

The main \emph{complexity measure} for proof-labeling schemes is the size of the certificates assigned to the nodes by the prover. The objective of the paper is to design schemes with logarithmic-size certificates, for two classes of graphs: the class~$\G^+_k$, $k\geq 0$, of graphs embeddable on an orientable closed surface of genus at most~$k$, and the class $\G^-_k$, $k\geq 1$, of graphs embeddable on a non-orientable closed surface of genus at most~$k$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Pierre : Sous-sous-section "Combinatorial Embedding" en commentaire car apparemment 
% non nÃ©cessaire. Si finalement nÃ©cessaire, Ã  rÃ©intÃ©grer, et je ferai une passe dessus. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsubsection{Combinatorial embedding}
% {\color{red} Cette section est elle utile ? }
% 
% 
% Given an embedding, the relative positions of  edges incident in any vertex $v$ are fixed by the embedding, and can be given by a cyclic permutation $\pi_v$ of these edges. The permutation $\pi_v$ has to be chosen according two inverse cyclic permutations of edges incident in $v$. Remark that if the embedding is done on an orientable surface, all permutations can be chosen in respecting the clockwise direction, while this has no sense if the embedding is done on an non-orientable surface.   
% 
% Two edges $ \{v,w \}$ and   $\{v,w' \}$ incident in $v$  are on the boundary of a same face if an only if either   
% $\{v,w' \} = \pi_v(\{v,w\})$ or   $\{v,w' \} = \pi_v^{-1}(\{v,w\})$. Moreover, for each face $f$ of a 2-cell embedding, a boundary walk of $f$ can be given by a path  $(v_0, v_1, ...,  v_{p-1}, v_p =  v_0)$  
%such that  $$ \{v_{i}\,v_{i+1} \} =  ( \pi_{ v_{i}})^{\lambda (\{v_i \, v_{i-1}\})} (\{v_{i}\,v_{i-1} \}). $$ 
%where $\lambda (\{v_i \, v_{i-1}\}) \in \{-1, 1\}$. 
%Informally, this means that the embedding is essentially given by permutations $\pi_v$ for all vertices,  and values $\lambda (\{v, w\})$ for all edges. This is the motivation of the definition below.  
%
%\begin{definition}
% A \emph{combinatorial embedding} is given by 
%\begin{itemize}
%\item for each vertex  $v \in V$,  a cyclic permutation $\pi_v$ of edges incident in $v$, (this set of permutation is called a \emph{rotation system}), 
%\item a \emph{signature} $\lambda : E \rightarrow \{-1, 1\}$. 
%\end{itemize}
%\end{definition}
%
%
%
%From a combinatorial embedding  some polygonal faces can be constructed,  using facial paths  $(v_0, v_1, ...,  v_{p-1}, v_p =  v_0)$  such that  $ \{v_{i}\,v_{i+1} \} =  ( \pi_{ v_{i}})^{\lambda (\{v_i \, v_{i-1}\})} (\{v_{i}\,v_{i-1} \}). $
%Afterward, faces can be glued according to edges to construct a topological compact surface. 
%
%\begin{proposition}\cite{Stahl78, Yo63}
%There exists a  2-cell embedding of  $G$ into $X$ if and only if there exists a combinatorial embedding of $G$  which constructs a topological surface homeomorphic to   $X$. 
%%In  particular, $(X, T)$ is a necessarily a compact surface.  
%
%Moreover, given a 2-cell embedding of $G$  into an orientable closed surface $X$, a combinatorial embedding of $G$ whose signature is uniformly equal to 1  can be canonically be deduced.%, the clockwise direction of edges around each vertex $v$  defining $\pi_v$. 
%
%Conversely,  for each combinatorial embedding of $G$ whose signature is uniformly equal to 1, the constructed closed surface is orientable, and  the clockwise direction  of edges around each vertex $v$ can be defined using $\pi_v$. 
%\end{proposition}
%
%




==> s3-duplication-old.tex <==
% !TEX root = main-PLS-surface.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Unfolding a Torus}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 In this section, we describe how to ``flat down'' a surface, by reducing it to a disk whose boundary has a specific form. This operation is central for constructing the distributed certificates in our proof-labeling scheme. In fact it provides a centralized certificate for bounded genus. The section is  dedicated to orientable surfaces, and the case of non-orientable surfaces will be treated further in the text. 
 
%-------------------------------------------------------------------------------------------------
\subsection{Separation and Duplication}
\label{G_C}
%-------------------------------------------------------------------------------------------------

Given a 2-cell embedding of a graph $G$ on a  closed  surface  $X$, a \emph{non-separating cycle}  of the embedding is a simple cycle $C$ in $G$ such that     $X \smallsetminus  C$ is connected.   Figure~\ref{fig:separating} illustrates this notion. For the red loop $C_1$ in $\T_1$ displayed on the left, $X \smallsetminus  C_1$ is connected, and therefore $C_1$ is non-separating. Instead, for the red loop $C_2$ in $\T_1$ displayed third from the left on  Figure~\ref{fig:separating}, $X \smallsetminus  C_2$ is disconnected, and therefore $C_2$ is separating. The result hereafter is a classical result, whose proof can be found in, e.g., \cite{mohar2001graphs,Ortner08}.     
 
\begin{figure}[tb]
\begin{center}
\begin{tabular}{cccc}
\includegraphics[scale=0.15]{figures/fig-separating-1.png}
&
\includegraphics[scale=0.15]{figures/fig-separating-2.png}
&
\includegraphics[scale=0.15]{figures/fig-separating-3.png}
&
\includegraphics[scale=0.15]{figures/fig-separating-4.png}
\end{tabular}
\end{center}
\caption{Separating and non-separating cycles}
\label{fig:separating}
\end{figure} 
 
 \begin{lemma} \label{first_cycle}
Let $G$ be a graph embeddable on a closed orientable surface $X$ with genus $k \geq 1$. For any 2-cell embedding of $G$ on $X$, there exists a non-separating cycle $C$ in $G$.  
 \end{lemma}
   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pierre : Preuve commentÃ©e car inutile puisque rÃ©sultat connu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %
% 
% \begin{proof} 
% The proof below is very close to the proof given in \cite{Ortner08}. 
% This is done as follows using the following transformation.  See Figure~\ref{fig:find-cycle}.
% \begin{itemize}
% \item   if an edge is shared between two distincts faces, then merge these two faces by deleting the edge (from the graph, and from the embedding) 
%\item  if there is a pending edge, then delete the edge and the corresponding vertex (from the graph, and from the embedding) 
%\end{itemize}
%
%Starting from  the embedding of $G$, and doing a sequence of such transformations,  a sequence of embeddings in $(X, T)$ of graphs $G_0, G_1, ..., G_p$ is obtained, with
%\begin{itemize}
%\item $G_0   = G$,
%\item for $0 \leq i < p$,  $G_{i+1}$  is deduced from $G_{i}$ by removing an edge, if the first item applies,  or an edge and an vertex when the second one applies,
%\item no transformation is possible in the embedding of $G_p$.
%\end{itemize}
%
%\begin{figure}[!h]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{center}
%\begin{tabular}{cccc}
%\includegraphics[scale=0.15]{figures/fig-find-cycle-1.png}
%&
%\includegraphics[scale=0.15]{figures/fig-find-cycle-2.png}
%&
%\includegraphics[scale=0.15]{figures/fig-find-cycle-3.png}
%&
%\includegraphics[scale=0.15]{figures/fig-find-cycle-4.png}
%\end{tabular}
%\end{center}
%\caption{\label{fig:find-cycle}}
%\end{figure} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%By construction, we  have  an embedding of $G_p$  on $X$ with a unique face.    Thus $X \setminus G_p$ is connected.  
%By construction also,  $G_p $ has no pending vertex. 
%Moreover $G_p$ is not reduced to a point  $v$, since,  otherwise,  its embedding would not be cellular: the unique face would be the set   $X \setminus \{v \}$, which  is not homeomorphic to an open disk, since $X$ is of genus al least $k \geq 1$. 
%Thus,  there exists a simple cycle $C$ in  $G_p$. The cycle $C$ is necessarily a non-separating  cycle of the embedding of $G_p$, and,  consequently, a non-separating  cycle of the embedding of $G$. 
% \end{proof}

\subsubsection{Cycle duplication} 

Let $G$ be a graph embeddable on a closed orientable surface $X$. Given a 2-cell embedding~$f$ of  $G$ on~$X$,  let $C$ be a non-separating orientable cycle of $G$ whose existence is guaranteed by Lemma~\ref{first_cycle}. By definition, the left and right sides of $C$ can be defined on the neighborhood of $C$. We denote by $G_C$ the graph obtained by \emph{duplication} of~$C$ in~$G$. Specifically, let $C = (v_0, \dots, v_r)$. Every vertex $w\notin C$ remains in $G_C$, as well as every edge non incident to a vertex of~$C$. Every vertex $v_i $ of $C$ is replaced by a left vertex~$v'_i$ and a right vertex~$v''_i $. For every $i=0,\dots,r-1$,  $\{v'_i, v'_{i+1} \} $  and $ \{v''_i, v''_{i+1} \} $ are  edges of $G_C$. Finally, for every $i=0,\dots,r$, and every neighbor $w\notin C$ of $v_i$ in $G$,  if $f( \{v_i, w \}) $  meets the left of $C$, then $\{v'_i,w\}$ is an edge of $G_C$, otherwise  $\{v''_i,w\}$ is an edge of $G_C$.  The embedding $f$ of $G$ on $X$ directly induces an embedding of $G_C $ on~$X$. Figure~\ref{fig:duplication-simple} illustrates the operation of duplication, and the resulting embedding. 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.3]{figures/fig-cycle-duplication-1.png}
\includegraphics[scale=0.3]{figures/fig-cycle-duplication-inter.png}
\includegraphics[scale=0.3]{figures/fig-cycle-duplication-2.png}}
\caption{Cycle duplication and the associated surface}
\label{fig:duplication-simple}
\end{figure}

The embedding of $G_C $ on~$X$ is however not a 2-cell embedding, as it contains the face $\phi$ between $C'$ and $C''$ on~$X$, where  $C'  = (v'_0, \dots, v'_r)$ and $C'' = (v''_0, \dots,v''_r)$. Formally, $\phi$ is the face with boundary $C'\cup C''$. Let $X_C$ be the surface obtained from $X$ by removing~$\phi$, and by replacing $\phi$ with two faces $\phi'$ and $\phi''$ with  boundary walks $C'$ and $C''$, respectively (see Figure~\ref{fig:duplication-simple}). The embedding $f$ of $G$ on $X$ induces a 2-cell embedding $f_C$ of $G_C$ on $X_C $.  Also, since $C$ is a non-separating cycle of  $G$ in $X$, the surface $X_C$ is path-connected. Moreover, as $X$ is orientable, $X_C$  is  also orientable. Indeed, every simple cycle of $X_C$ not intersecting $\phi'$ nor $\phi''$ is a cycle of $X$, and  is therefore orientable. Furthermore, any simple cycle of $X_C$ intersecting $\phi'$ and/pr $\phi''$ is homotopic to a cycle separated from both boundaries of $\phi'$ and $\phi''$ by an open set, and thus is homotopic to a cycle of~$X$. It follows that  $X_C$ is a closed orientable surface, and thus, thanks to Lemma~\ref{euler}, the genus of $X_C $  is~$k-1$. 

\subsubsection{Path duplication} 

Again, let us consider a graph $G$, an orientable closed surface~$X$, and a 2-cell embedding $f$ of   $G$ on  $X$. Let $\phi, \psi$ be two distinct faces of the embedding, and let $ P =   (w_0, \dots, w_r)$  be simple path (possibly reduced to a single vertex) between $\phi$ and $\psi$ (see Figure~\ref{fig:path-duplication-simple}). That is, $P$ is such that  $w_0 $ is on the boundary of  $\phi$, $w_r $ is on the boundary of  $\psi$, and no  intermediate vertex $w_i$, $0 < i < r$,  is  in the boundary of $\phi$ or~$\psi$.  The path~$P$ enables to define a graph  $G_{ P}$ obtained by duplicating the path $P$ in a  way similar to the way the cycle $C$ was duplicated in the previous section. There is only one subtle difference, as the left and right side of the path cannot be defined at its endpoints. Nevertheless, left and right can still be properly defined by virtually extending the path so that it ends up in the interiors  of $\phi$ and $\psi$.  Thanks to path duplication, the two faces $\phi$ and $\psi$ of $G$ are replaced by a unique face of $G_P$ as illustrated on Figure~\ref{fig:path-duplication-simple}, reducing the number of faces by one.  

\begin{figure}[tb]
\begin{center}
\includegraphics[scale=0.3]{figures/pierre-1.png}
\includegraphics[scale=0.3]{figures/pierre-2.png}
\caption{Path duplication. }
\label{fig:path-duplication-simple} 
\end{center}
\end{figure} 

\paragraph{Remark.} 

Cycle duplication and path duplication are typically used conjointly. A basic example, used for the torus~$\T_1$ in the next section, consists of, first, duplicating a cycle~$C$, then connecting the two faces resulting from this duplication by a path~$P$, and, finally, duplicating~$P$ for merging these two faces into one single face. 
%The corresponding graph is denoted by $G_{C,P}$. 
Further, for the general case $\T_k$, $k\geq 1$,  $k$~cycles are duplicated, and  $2k-1$ duplicated paths  connect these cycles for unfolding the surface. 

\begin{figure}[!h]
\begin{center}
\begin{tabular}{cc}
\includegraphics[scale=0.25]{figures/fig-K33-torus.png}
\end{tabular}
\caption{$K_{3,3}$ embedded on the torus.}
\label{fig:K33-torus-paths1} 
\end{center}
\end{figure}

%-------------------------------------------------------------------------------------------------
\subsection{Unfolding the Torus $\T_1$}
\label{subsec:cas-du-tore}
%-------------------------------------------------------------------------------------------------

Let $G$ be a graph, and let $f$ be a 2-cell embedding of $G$ on~$X=\T_1$ --- see Figure~\ref{fig:cut-pierre}(a) for an embedding of $K_5$ on $\T_1$, as an illustrative example. Let $C=(v_0,\dots,v_r)$ be a non-separating orientable cycle of $G$, e.g., the cycle $(a,b,c)$ on Figure~\ref{fig:cut-pierre}(a)). Let 
$
C'=(v'_0,\dots,v'_r) \; \mbox{and} \; C''=(v''_0,\dots,v''_r)
$
be the two cycles resulting from the duplication of~$C$, e.g., the cycles $(a',b',c')$ and $(a'',b'',c'')$ on Figure~\ref{fig:cut-pierre}(b). Thanks to Lemma~\ref{connect}, the graph $G_C$ with two new faces $\phi'$ and $\phi''$ is connected. Thus, in  particular, there exists  a simple path  $ P =   (w_0,  \dots, w_s)$  in $G_C$ from a vertex $v'_i\in C'$  to a vertex $v''_j\in C''$, such that every  intermediate vertex $w_i$, $0 < i < s$,  is not  in $C'\cup C''$, e.g. the path $(c'',d,b')$ on Figure~\ref{fig:cut-pierre}(b). Note that it may be the case that $i\neq j$. On Figure~\ref{fig:cut-pierre}(b), the path $(b'',e,d,b')$ satisfies $i=j$, but Figure~\ref{fig:K33-torus-paths1} illustrates an embedding of $K_{3,3}$ on $\T1$ for which $i=j$ cannot occur. Duplicating $P$ enables to obtain a graph $G_{C, P}$ with only a special face $\phi$,  whose boundary contains all duplicated vertices and only them (see Figure~\ref{fig:cut-pierre}(c)). The details of the vertex-duplications, and of the edge-connections are detailed hereafter. 
 
\begin{figure}[tb]
\centerline{\includegraphics[scale=0.15]{figures/pierreK55.jpg}}
\caption{Unfolding $K_5$ embedded on the torus $\T_1$. }
\label{fig:cut-pierre} 
\end{figure} 

Let $ P' =   (w'_0,  \dots, w'_s)$ and $ P'' =   (w''_0,  \dots, w''_s)$ be the two paths obtained by duplicating~$P$. In particular, the vertices $w_0=v'_i$ and $w_s = v''_j$ are both duplicated in $w'_0, w''_0$,  and  $w'_s, w''_s$, respectively. The edges 
\[
\{v'_{i-1},v'_i\}, \; \{v'_i,v'_{i+1}\}, \; \{v''_{j-1},v''_j\}, \; \mbox{and} \; \{v''_j,v''_{j+1}\}
\] 
are  replaced by the edges connecting $v'_{i-1},v'_{i+1},v''_{j-1},v''_{j+1}$ to $w'_0, w''_0, w'_s,w''_s$.  For defining these edges, observe that the path $P$ in $\T_1$ induces a path $Q =   (v_i,  w_1,\dots, w_{s-1}, v_j)$ in $G$  connecting the vertices $v_i$ and $v_j$ of~$C$,  such that, in the embedding on~$\T_1$, the edge  $\{v_i,  w_1\}$ meets $C$ on one side while the edge  $\{w_{s-1}, v_j\}$  meets $C$  on the other side (see Figure~\ref{fig:cutpathQ}). 

\begin{figure}[htb]
\centerline{\includegraphics[scale=0.23]{figures/pierre-3.png}}
\caption{Orienting the edges at the two extremities of the path}
\label{fig:cutpathQ} 
\end{figure} 

\noindent Let us assume, w.l.o.g., that  the edges of $C \cup Q$ around $v_i$ are in the order 
\[
\{v_i, v_{i-1} \}, \; \{v_i, v_{i+1}\}, \; \{v_i, w_1 \}
\]
when visited clockwise in~$\T_1$. It follows that the edges of $C \cup Q$ around $v_j$ are in the order 
\[
 \{v_j, v_{j-1} \},  \{v_j, v_{j+1}\},  \{v_j, w_{s-1} \} 
 \]
 when visited counter-clockwise in~$\T_1$. These orders are transferred in~$G_C$, that is, the edges of $C' \cup P$ around $v'_i$ are in clockwise order 
 \[
  \{v'_i, v'_{i-1} \},   \{v'_i, v'_{i+1} \}, \{v'_i, w_{1} \}, 
  \]
  while the edges of $C'' \cup P$ around $v''_j$ are in counter-clockwise order 
  \[
  \{v''_j, v''_{j-1} \},  \{v''_j, v''_{j+1}\}, \{v''_j, w_{s-1} \}.
  \] 
  This guarantees that $v'_{i-1}$ and $v''_{j-1}$ are in the same side of the path $P$. More generally,  the relative positions of $v'_{i-1}$, $v'_{i+1}$,  $v''_{j-1}$, and  $v''_{j+1}$ w.r.t.~$P$ are as follows.  Vertices $v'_{i-1}$ and $v''_{j-1}$  are on the same side of~$P$, while vertices $v'_{i+1}$ and $v''_{j+1}$ are on the other  side of~$P$.  As a consequence, it can be assumed that, in the graph $G_{C, P}$ resulting from the duplications of both~$C$ and~$P$, the vertices $v'_{i-1}$ and $v''_{j-1}$ are connected to the end points of~$P'$,  while $v'_{i+1}$ and $v''_{j+1}$ are connected to the end points of~$P''$.  It follows that  
  \[
  \{w'_0, v'_{i-1} \}, \{w'_s, v''_{j-1} \}, \{w''_0, v'_{i+1} \}, \mbox{and} \; \{w''_s, v''_{j+1} \}
  \]
  are edges of $G_{C, P}$.  

The embedding $f$ of $G$ on $X=\T_1$ directly induces an embedding of $H^*=G_{C, P}$ on~$X_C$, as illustrated on Figure~\ref{fig:cut-pierre}(d). As observed before, the genus of $X_C$ is one less than the genus of~$X$. Since $X=\T_1$, it follows that the embedding $f$ of $G$ on $\T_1$  actually induces a planar embedding $f^*$ of $H^*$.  The faces of this embedding are merely the faces of $G$,  plus another, special, face $\phi^*$ whose boundary walk is 
\begin{align}
B^*= (w'_0, w'_1, \dots, w'_s, & v''_{j-1}, v''_{j-2}, \dots, v''_0,v''_r,\dots,v''_{j+1},  \label{eq:boundwalk}\\
& w''_s, w''_{s-1} , \dots, w''_0, v'_{i+1}, v'_{i+2},\dots,v'_r,v'_0,\dots, v'_{i-1}) \nonumber
\end{align}
On Figure~\ref{fig:cut-pierre}(d), $B^*=(b'_1,d_1,c''_1,a'',b'',c''_2,d_2,b'_2,a',c')$. Our interest for $H^*,f^*,\phi^*$, and $B^*$ as far as the design of proof-labeling scheme is concerned resides in the fact that, as shown hereafter, they form a (centralized) certificate for genus~1. To see why, let us first define the notion of  \emph{splitting}. 

\begin{definition}\label{def:splitting}
A graph $H$ is a \emph{splitting}  of a graph $G$ if there exists a partition $(S_v)_{v \in V(G)}$ of~$V(H)$ such that:
\begin{enumerate}
\item \label{item:splitting-no-new-edge} 
For every $\{a,b\} \in E(H)$, if  $a\in S_u$ and  $b\in S_v$ with $u\neq v$, then $\{u,v\}\in E(G)$;
\item \label{item:splitting-every-old-edge}
For every $\{u,v\} \in E(G)$, there exists $\{a,b\}\in E(H)$ such that $a\in S_u$ and $b\in S_v$.
\end{enumerate}
The \emph{degree} of a splitting $H$ of $G$ is $\max_{v\in V(G)}|S_v|$, and $H$ is then said to be a $d$-splitting of~$G$.  
% A splitting is \emph{connected}, if, for every~$v\in V(G)$, the subgraph of $H$ induced by~$S_v$ is connected.  
\end{definition}

Intuitively, in a splitting~$H$ of~$G$, for every  vertex~$u$ of $G$ such that $ \vert S_u \vert = 1$,  it can be assumed, w.l.o.g.,  that $ S_u = \{ u \}$, abbreviated in $u\rightarrow \{u\}$. The fact that  the $|S_u| > 1$ indicates that vertex~$u$  is split in $H$ into several copies $u_1,\dots,u_\ell$ for some $\ell>1$, which form the nodes in~$S_u\subseteq V(H)$, abbreviated in $u\rightarrow \{u_1,\dots,u_\ell\}$. A vertex $u$ of $G$ such that $|S_u| > 1$ is thus said to be \emph{split}
in~$H$. The structure of the subgraph of~$H$ induced by $S_u$ is not specified.  Condition~\ref{item:splitting-no-new-edge} just states that if there is an edge between two vertices $a$ and $b$ of $H$ then either $a$ and $b$ are copies of the same vertex~$u$ of~$G$, or they are the respective copies of two neighboring vertices $u$ and~$v$ in~$G$.  Condition~\ref{item:splitting-every-old-edge} states that every edge $\{u,v\}$ of $G$ must induce at least one edge of $H$ between a  copy of $u$ and a copy of~$v$.

Let $H$ be a splitting of a graph~$G$, let $f$ be a planar embedding of~$H$, and let~$\Phi$ be a face of~$H$ embedded on~$\T_0$. Let 
$
B=(u_0,\dots,u_N)
$
be a boundary walk of $\phi$. We say that $B$ is \emph{historically consistent} if all split vertices of $G$ in~$H$ are on~$B$, and if there exists vertices $v'_0,\dots,v'_r$, $v''_0,\dots,v''_r$, $w'_0, \dots, w'_s$, $w''_0, \dots, w''_s$ of~$H$ such that 
\[
B= (w'_0, \dots, w'_s,  v''_{j-1},  \dots, v''_0,v''_r,\dots,v''_{j+1}, 
w''_s,  \dots, w''_0, v'_{i+1},\dots,v'_r,v'_0,\dots, v'_{i-1}) 
\]
where 
\begin{itemize}
\item for every $k\in\{1,\dots,s-1\}$, $w'_k$ and $w''_k$ are split of a same vertex~$w_k$ of~$G$, 
\item for every~$k\in\{0,\dots,r\}\smallsetminus \{i,j\}$, $v'_k$ and $v''_k$ are split of a vertex~$v_k$ of~$G$, and
\item if $i\neq j$ then $w'_0,w''_0,v''_i$ are split of a vertex~$v_i$ of~$G$ while $w'_s,w''_s,v'_j$ are split of another vertex~$v_j$ of~$G$, otherwise $w'_0,w''_0,w'_s,w''_s$ are split of a same vertex~$v_i$ of~$G$. 
\end{itemize} 
By construction, the boundary walk $B^*$ of $\phi^*$ displayed in Eq.~\eqref{eq:boundwalk}  is historically consistent. The following result is specific of the torus, but it illustrates the basis for the design of our proof-labeling schemes. 
 
\begin{lemma}\label{lem:certif-T1-centralized}
Let  $H$ be a splitting of a graph   $G$, and assume that there exists a planar embedding~$f$ of $H$ with a face $\phi$  such that its boundary walk $B$ is historically consistent. Then $G$ can be embedded in the torus~$\T_1$.
\end{lemma}

\begin{proof}
Using the specifications of the splits, the two sub-paths $(w'_0, \dots, w'_s)$ and  $(w''_0, \dots, w''_s)$ of~$B$ can be identified by merging each pair of nodes $w'_i$ and $w''_i$, $i\in\{0,\dots,s\}$, into a single node~$w_i$, for forming a single path. The face~$\phi$ of the planar embedding~$f$ of $H$ can be replaced by two faces $\phi'$ and $\phi''$, with respective boundary walks $(v'_0,v'_1,\dots, v'_r)$ and  $(v''_r, v''_{r-1},\dots, v''_0)$ with vertices ordered clockwise. These transformations preserve the planarity of the embedding. Next, the two cycles $(v'_0,\dots, v'_r)$ and  $(v''_0, \dots, v''_r)$ can be identified, by merging each pair of nodes $v'_i$ and $v''_i$ into~$v_i$. As a result, the two faces $\phi'$ and $\phi''$ are replaced by a handle, providing an embedding of $G$ on~$\T_1$.
\end{proof}

The outcome of the lemma is that $(H^*,f^*,\phi^*,B^*)$ is a certificate that $G$ can be embedded in~$\T_1$. In the next section, we show how to generalize this construction for deriving a certificate that a graph $G$ can be embedded in~$\T_k$, $k>1$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Unfolding $\T_k$ for $k\geq 1$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The process described in the previous section for genus~1 can be generalized to larger genus $k\geq 1$, as follows. Again, let $G$ be a graph, and let $f$ be a 2-cell embedding of $G$ on~$T_k$. 

%--------------------------------------------------------------------------------------------------------
\subsection{The face-duplication phase}
%--------------------------------------------------------------------------------------------------------

Let $X^{(0)}=\T_k$. As for the torus, let $C_1$ be a non-separating orientable cycle of $G^{(0)}=G$, and let us consider the embedding of $G^{(1)}=G^{(0)}_{C_1}$  induced by~$f$, on  the  surface $X^{(1)}=X^{(0)}_{C_1}$ of genus~$k-1$. This operation can be repeated. Indeed, by Lemma~\ref{first_cycle}, there exists a non separating cycle $C_2$ of  $G^{(1)}$. The graph $G^{(2)}=G^{(1)}_{C_2}$ can be embedded on the surface $X^{(2)}=X^{(1)}_{C_2} $ with one face more than the number of faces of the embedding of $G^{(1)}$ on  $X^{(1)}$, and thus two more  faces than the number of faces of the embedding of $G$ on  $\T_k$. By Lemma~\ref{euler}, $X^{(2)}$ has thus genus~$k-2$. See Figure~\ref{fig:pierreT2}(a-b). 

This process can actually be iterated  $k$ times, resulting in a sequence of $k+1$ graphs $G^{(0)}, \dots, G^{(k)}$ where $G^{(0)}=G$, and a sequence of $k+1$ closed surfaces $X^{(0)}, \dots, X^{(k)}$ where $X^{(0)}=\T_k$. Each graph $G^{(i)}$ is embedded on the closed surface $X^{(i)}$ of genus~$k-i$, as follows. The embedding  of $G^{(0)}$ on $X^{(0)}$ is the embedding of $G$ on $X$, and, for every $i=0,\dots,k-1$,  the embedding of $G^{(i+1)}$ on $X^{(i+1)}$ is induced by the embedding of $G^{(i)}$ on $X^{(i)}$, after duplication of a non-separating cycle~$C_{i+1}$ of $G^{(i)}$ into two cycles $C'_{i+1}$ and $C''_{i+1}$. 

The closed surface $X^{(k)}$ is of genus~0, i.e.  $X^{(k)}$ is homeomorphic to the sphere $\T_0 = S^2$ (see  Figure~\ref{fig:pierreT2}(b)). The graph  $G^{(k)}$ is therefore planar, for it contains $k$ more faces  than the number of faces in~$G$, as two new faces $\phi'_i$ and $\phi''_i$ are created at each iteration~$i$, in replacement to one face $\phi_i$, for every $i=1,\dots,k$.   

\begin{figure}[htb]
\centerline{\includegraphics[scale=0.15]{figures/pierreT2.jpg}}
\caption{A simple unfolding of a graph $G$ embedded on $\T_k$}
\label{fig:pierreT2} 
\end{figure} 

%--------------------------------------------------------------------------------------------------------
\subsection{The face-reduction phase}
%--------------------------------------------------------------------------------------------------------

The objective is now to replace the $2k$ faces $\phi'_i,\phi''_i$, $i=0,\dots,k-1$, by a single face. For this purpose, let's relabel these faces as $\psi_1,\dots,\psi_{2k}$ is arbitrary order (see Figure~\ref{fig:pierreT2}(c)). Let $\chi_1=\psi_1$. There exists a simple path~$P_1$ between the two  faces  $\chi_1$ and $\psi_2$.  Duplicating $P_1$ preserves the fact that the  graph $G^{(k+1)}=G^{(k)}_{P_1}$ can be embedded on the sphere~$\T_0$.  By this duplication, the two faces $\chi_1$ and $\psi_2$ are merged into a single face $\chi_2$. Now, there is a simple path~$P_2$ between the two  faces  $\chi_2$ and $\psi_3$ (see Figure~\ref{fig:pierreT2}(d)).  Again, duplicating $P_2$ preserves the fact that the  graph $G^{(k+2)}=G^{(k+1)}_{P_2}$ can be embedded on the sphere~$\T_0$, in which the two faces $\chi_2$ and $\psi_3$ are now merged into a single face $\chi_3$. By iterating this process, a finite sequence of graphs $G^{(k)},\dots, G^{(3k-1)}$ is constructed, where, for $i=0,\dots,2k-1$, the graph $G^{(k+i)}$ is coming with its embedding on~$\T_0$, and with a set of special faces $\chi_{i+1},\psi_{i+2},\dots,\psi_{2k}$. A path $P_{i+1}$ between $\chi_{i+1}$ and $\psi_{i+2}$ is duplicated for merging these two faces into a single face~$\chi_{i+2}$, while preserving the fact that $G^{(k+i+1)}=G^{(k+i)}_{P_{i+1}}$ can be embedded on the sphere~$\T_0$. 
 
Eventually, the process results in a single face $\phi^*=\chi_{2k}$ of $H^*=G^{(3k-1)}$ (see Figure~\ref{fig:pierreT2}(e)). This face contains all duplicated vertices. The embedding $f$ of $G$ in $\T_k$ induces a planar embedding of $H^*$ whose external face~$\phi^*$ (see Figure~\ref{fig:pierreT2}(f)). 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.15]{figures/pierreT2-complex.jpg}}
\caption{A more complex unfolding a graph $G$ embedded on $\T_k$}
\label{fig:pierreT2-complex} 
\end{figure} 

%--------------------------------------------------------------------------------------------------------
\subsection{Certifying genus at most~$k$}
%--------------------------------------------------------------------------------------------------------

Conversely, an embedding of  $G$ in $\T_k$ can be  induced from the embedding $f^*$ of $H^*$ on $\T_0$, and from the boundary walk~$B^*$  of~$\phi^*$. The latter is indeed entirely determined  by the successive cycle- and path- duplications performed during the whole process. It contains all duplicated vertices, resulting from the cycles $C'_1,\dots ,C'_k$ and $C''_1,\dots ,C''_k$, and from the paths $P'_1, \dots, P'_{2k-1}$ and $P''_1, \dots, P''_{2k-1}$.  Note that the duplication process for a vertex may be complex. A vertex may indeed be duplicated once, and then one of its copies may be duplicated again, and so on, depending on which cycle or path is duplicated at every step of the process.  This phenomenon actually already occurred in the basic case of the torus~$\T_1$ where the duplications of $v_i$ and $v_j$ were more complex that those of the other vertices, and were also differing depending on whether $i=j$ or not. Figure~\ref{fig:pierreT2-complex} illustrates a case in which two cycles $C_i$ and $C_j$ share vertices and edges in $\T_2$, causing a series of duplication more complex than the basic case illustrated on Figure~\ref{fig:pierreT2}. In particular, a same vertex of $H^*$  may appear several times the boundary walk $B^*$, and a same edge of $H^*$ may be traversed twice, once in each direction.  

The successive duplications experienced by a vertex~$v$ of the actual graph $G$ during the face-duplication and face-reduction phases can be encoded as a rooted binary tree unfolding these duplications, called \emph{history}. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Histories}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

For every vertex~$v$ of~$G$, the history of~$v$ is denoted by~$\hist(v)$. Figure~\ref{fig:cut-arbre2} displays the general structure of the history~$\hist(v)$ of a node~$v$. In the rooted binary tree~$\hist(v)$, all edges are labeled. Specifically, for a graph~$G$ of genus~$k$, the label of an edge in a history is taken from the set 
\[
\mathcal{L}_k=\{C'_1,\dots ,C'_k,C''_1,\dots ,C''_k,P'_1, \dots, P'_{2k-1},P''_1, \dots, P''_{2k-1}\}.
\] 
It is required that the two edges connecting a node~$\hist(v)$ to its two children have labels $C'_i$ and $C''_i$, for some $i\in\{1,\dots,k\}$, or labels $P'_i$ and $P''_i$, for some $i\in\{1,\dots,2k-1\}$. Furthermore, the edge-labels must respect an order (reflecting the order in which the different duplications takes place). Specifically, for any shortest path $e_1,\dots,e_t$ from the root to a leave of~$\hist(v)$, the corresponding sequence of labels is of the form 
\[
C_{i_1},\dots,C_{i_r},P_{j_1},\dots,P_{j_s}
\]
where the prime and double-prime symbols are omitted, with $r\geq 0$, $s\geq 0$, $1\leq i_1 < \dots < i_r\leq k$, $1\leq j_1 < \dots < j_s\leq 2k-1$, and $r+s=t$. A node of $\hist(v)$ whose incident edge leading to the root is labeled $C'_i$ (resp., $C''_i,P'_i,P''_i$) is of \emph{type} $C'_i$ (resp., $C''_i,P'_i,P''_i$). 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.12]{figures/history2.jpg}}
\caption{History of a node $v$ in $\T_k$.}
\label{fig:cut-arbre2} 
\end{figure} 

In addition, for every vertex~$v$ of $G$, every leaf of $\hist(v)$ is labeled by the vertex $y$ of $H^*$ corresponding to the duplication experienced by~$v$ according to the labels of the path from the root of $\hist(v)$ to the considered leaf. In particular, a history $\hist(v)$ with no edges has its unique node labeled~$v$ itself. Figure~\ref{fig:cut-arbre} displays the histories of $v_i$ and $v_j$ corresponding to the case of a graph~$G$ embedded on the torus~$\T_1$, as described in Section~\ref{subsec:cas-du-tore}, depending on whether $i=j$ or not. 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.12]{figures/history-simple.jpg}}
\caption{Partial histories in the case of $\T_1$}
\label{fig:cut-arbre} 
\end{figure} 

In fact, for the objective of determining an embedding of $G$ in $\T_k$ given a planar embedding $f*$ of $H^*$, the histories are provided additional information. Let us provide the boundary walk $B^*$ of $\phi^*$ with a direction, say clockwise. For $v\in V(G)$, every leaf of $\hist(v)$ is not only labeled by the vertex $y\in V(H^*)$ corresponding to the duplications of $v$ specified by the edge-labels of the path from the root of $\hist(v)$ to this leaf, but also by a collection of triples of vertices of $H^*$, of the form $(x,y,z)$ where $x,y,z$ are vertices of $H^*$, and $y$ is the split of $v$ 	as specified by the edge-labels along the path from the root of $\hist(v)$ to the leaf. The node $x$ is the predecessor of $y$ along the boundary walk $B^*$ traversed clockwise, and $z$ is its successor. Since $y$ may appear several times on $B^*$, the leaf is labeled by a collection $\{(x_1,y,z_1),\dots,(x_\ell,y,z_\ell)\}$ for some $\ell\geq 1$, corresponding to the $\ell$ times that vertex $y$ is encountered when traversing $B^*$ in the clockwise direction. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Filling up histories}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

Given the history $\hist(v)$ of a vertex $v\in V(G)$, there is a canonical way to automatically provide the internal nodes with labels. Let us respectively denote by 
\[
x \xrightarrow{C_i} \{x',x''\}, \; x \xrightarrow{P_i} \{x',x''\}, \; x \xrightarrow{C_i} \{x\}, \; \mbox{and} \; x \xrightarrow{P_i} \{x\} 
\]
the fact that vertex $x$ is split in $x'$ and $x''$ when $C_i$ is duplicated, 
the fact that vertex $x$ is split in $x'$ and $x''$ when $P_i$ is duplicated, 
the fact that vertex $x$ remains untouched when $C_i$ is duplicated, and 
the fact that vertex $x$ remains untouched when $P_i$ is duplicated.
We sometime adopt compact notations like 
\[
x|y \xrightarrow{C_i} \{x',x''\}|\{y',y''\} 
\]
for stating that $x \xrightarrow{C_i} \{x',x''\}$ and $y \xrightarrow{C_i} \{y',y''\}$. 
Similarly, we denote by 
\[
L' \; L'' \xrightarrow{C_i} L, \; \mbox{(resp., } \; L_1 \; L_2 \xrightarrow{P_i} L_3)
\]
the fact that two twin nodes of type $C'_i$ and $C''_i$ (resp., $P'_i$ and $P''_i$), respectively labeled $L'$ and~$L''$, generate the label $L$ at their parent. Every history can then be filled up with labels by proceeding upwards, from leaves to root, according to the following \emph{fill up rules}:
\[
\left\{\begin{array}{ll}
(x',y',z') (z'',y'',x'') \xrightarrow{C_i} \bot & 
	\mbox{if} \;  \; x | y | z \xrightarrow{C_i}\{x',x''\}|\{y',y''\}|\{z',z''\};\\
%
(x',y',z') (z'',y'',x'') \xrightarrow{P_i} \bot & 
	\mbox{if} \; \; x | y | z \xrightarrow{P_i}\{x',x''\}|\{y',y''\}|\{z',z''\};\\
%
(x',y',z') (z'',y'',x'')  \xrightarrow{P_i} (x',y,x'') &
	\mbox{if}  \;\; x'|x''|y|z \xrightarrow{P_i} \{x'\} | \{x''\} | \{y',y''\} |  \{z',z''\}; \\
%
(x',y',z') (z'',y'',x'')  \xrightarrow{P_i}  (x',y,x'')\; ; (z'',y,z') &
	\mbox{if} \; \; x'|x''|y|z'|z'' \xrightarrow{P_i} \{x'\} | \{x''\} | \{y',y''\} | \{z'\} | \{z''\};\\
%
(x',y',z') (*,y'',*)  \xrightarrow{C_i|P_i}  (x',y,z') &
	\mbox{otherwise, where $y \xrightarrow{P_i} \{y',y''\}$.}  
\end{array}\right.
\]
Figure~\ref{fig:cut-arbre-consistent}  displays the filled up histories for the case of the torus $\T_1$ detailed in Section~\ref{subsec:cas-du-tore}. The first rule corresponds to the ``basic'' case of cycle duplication. Note that the two triples $(x',y',z')$ and $(z'',y'',x'')$ are ordered in opposite directions. This matches the requirement for correctly glueing the border of two faces in order to create a handle (see Figures~\ref{fig:hcc} and~\ref{fig:duplication-simple}). 

The second rule also corresponds to a ``basic'' case, for path duplication, but it is dedicated to the internal nodes of the path only. Also in this case, the two triples $(x',y',z')$ and $(z'',y'',x'')$ are ordered in opposite directions, to match the way the two copies of the path $P_i$ are traversed when traversing the boundary walk $B^*$ in clockwise direction (cf. Eq.~\eqref{eq:boundwalk} and Figure~\ref{fig:path-duplication-simple}). 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.15]{figures/history-consistent.jpg}}
\caption{The histories in the case of $\T_1$}
\label{fig:cut-arbre-consistent} 
\end{figure} 

The third rule also refers to path duplication, but dedicated to the extremities of the path (see Figures~\ref{fig:path-duplication-simple} and~\ref{fig:cut-arbre-consistent}). The fourth rule handles the pathological case in which the path connecting two faces is reduced to a single node~$y$ (i.e., the two corresponding cycles share at least one vertex~$y$). Then, as illustrated on Figure~\ref{fig:pathological}, only the vertex~$y$ is split during the path duplication, while its four neighbors $x,z,u$, and $w$ remain intact. 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.15]{figures/pathological.jpg}}
\caption{The case of a path $P_i$ reduced to a single node}
\label{fig:pathological} 
\end{figure} 

Finally, the fifth and last rule applies in the case one of the twin nodes carries a label $(x',y',z')$ (resp., $(x'',y'',z'')$) for which none of the labels $(z'',y'',x'')$ (resp., $(x',y',z')$) carried by its twin enable any of the fist four rules to apply. This may for instance result from the case of a path connecting two faces reduced to a single vertex, as illustrated on Figure~\ref{fig:pathological} which yields the tree displayed on Figure~\ref{fig:pathological-tree}. In this tree, the triple $(x',y,x'')$ cannot be matched, while the triple $(z'',y',z')$ can be matched with the triple $(\bar{z}',\bar{y},\bar{z}'')$ of its twin. 

\begin{figure}[tb]
\centerline{\includegraphics[scale=0.1]{figures/pathological-tree.jpg}}
\caption{A branch of a history resulting from the example of Figure~\ref{fig:pathological} }
\label{fig:pathological-tree} 
\end{figure} 

We have now all the ingredients to states what will be proved as sufficient to certify that a graph $G$ has genus at most~$k$. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Historical consistency}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

Let  $H$ be a splitting of a graph $G$, let~$f$  be a planar embedding of $H$, and let $\phi$ be a face of $H$ with  boundary walk $B$ directed, say, clockwise. The directed boundary walk~$B$ is denoted by~$\vec{B}$. Let 
$
\hist(G)=\{\hist(v),v\in V(G)\}
$
be a collection of histories for the vertices of~$G$, with edge-label in $\mathcal{L}_k$ for some $k\geq 1$. The collection $\hist(G)$ is \emph{consistent} with respect to $(G,H,\vec{B})$  if the following holds. 

%here exists a sequence of graphs $U_0,\dots,U_{3k-1}$ satisfying 
%\[ U_0=G, \;\; U_{3k-1}=H, \; \;\mbox{and $U_{i+1}$ is a splitting of $U_i$ for every $i=0,\dots,3k-2$}\]

\begin{enumerate}
\item \pierremp{What does mean ``successfully applied'' precisely?}
The fill up rules can be successfully applied to all trees of $\hist(G)$, and they result in all roots labeled~$\bot$. 

\item The collection of node-labels at the leaves of the histories in $\hist(G)$ can be ordered as $(x_0,y_0,z_0),\dots,(x_N,y_N,z_N)$ such that,  $y_i=z_{i-1}=x_{i+1}$ for every $i=0,\dots,N$, and $\vec{B}=(y_0,\dots,y_N)$.

\item For every $i=1,\dots,2k-1$, the collection of node-labels of the nodes of type $P'_i$ (resp.,~$P''_i$)  resulting from the fill up rules  can be ordered as $(x'_0,y'_0,z'_0),\dots,(x'_{s_i},y'_{s_i},z'_{s_i})$ (resp., $(z''_0,y''_0,x''_0),\dots,(z''_{s_i},y''_{s_i},x''_{s_i})$) for some $s_i\geq 0$ such that:

\begin{enumerate}
\item for every $j=0,\dots,s_i$, $y_j \xrightarrow{P_i} \{y'_j,y''_j\}$; 
\item for every $j=1,\dots,s_i$, $y'_j=z'_{j-1}$ and $y''_j=z''_{j-1}$; 
\item for every $j=0,\dots,s_i-1$, $y'_j=x'_{j+1}$ and $y''_j=x''_{j+1}$. 
\end{enumerate}

\item For every $i=1,\dots,k$, the collection of node-labels of the nodes of type $C'_i$ (resp.,~$C''_i$)  resulting from the fill up rules  can be ordered as $(x'_0,y'_0,z'_0),\dots,(x'_{r_i},y'_{r_i},z'_{r_i})$ (resp., $(z''_0,y''_0,x''_0),\dots,(z''_{r_i},y''_{r_i},x''_{r_i})$)  for some $r_i\geq 2$  such that:

\begin{enumerate}
\item for every $j=0,\dots,r_i$, $y_j \xrightarrow{C_i} \{y'_j,y''_j\}$; 
\item for every $j=0,\dots,s_i$, $y'_j=z'_{j-1}=x'_{i+1}$ and $y''_j=z''_{j-1}=x''_{i+1}$, where the arithmetic operations are taken modulo $r_i+1$. 
\end{enumerate}

\item \pierre{The unfolding satisfies $\chi_j,\psi_{j+1},\dots,\psi_{2k}$}
\end{enumerate}
By construction, the history $\hist^*(G)$ produced by encoding the unfolding the embedding of $G$ on $\T_k$ is  consistent w.r.t.~$(G,H^*,\vec{B}^*)$. 

% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 
\subsubsection{Centralized certification}
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - 

We are now ready to present a way to certify the fact that a graph has genus at most~$k$, in a centralized manner. 

\begin{theorem}\label{theo:certif-Tk-centralized}
Let  $H$ be a splitting of a graph $G$, let $f$ be a planar embedding of $H$, let $\phi$ be a face of $H$ with boundary walk $B$, and let $\hist(G)$ be an history of $G$ that is consistent w.r.t.~$(G,H,\vec{B})$ for some direction $\vec{B}$ of~$B$. Then $G$ can be embedded in~$\T_k$.
\end{theorem}

\begin{proof}
\pierre{to be done to be done to be done to be done to be done to be done to be done}
%
%The goal is to construct an explicit embedding of $G$ in~$\T_k$. Let us denote by 
%\[
%B_0=B=(u_0,\dots,u_N)
%\]
%the boundary walk of $\phi$, with $u_0=u_N$. The indices reflects a given orientation of the walk, say clockwise. Thanks to the histories of the nodes, one can identify the paths
%\[
%P'_{2k-1}=(w'_0, \dots, w'_s), \;\mbox{and} \; P''_{2k-1}=w''_0, \dots, w''_s 
%\]
%in $B_0$, namely 
%\[
%B_0=(u_0,\dots,u_\ell,w'_0, \dots, w'_s,u_{\ell+s+1},\dots,u_m,w''_s,\dots,w''_0,u_{m+s+1},\dots,u_N)
%\]
%for some indexes $\ell$ and $m$ with $m\geq \ell+s$. Identifying the nodes $w'_i$ and $w''_i$ into a node $w_i$ for every $i=0,\dots,s$, and removing the interior nodes $w_1,\dots,w_{s-1}$ of the resulting path, results in splitting $B_0$ into two sub-walks
%\[
%(u_0,\dots,u_\ell,w_0,u_{m+s+1},\dots,u_N), 
%\;\mbox{and} \; 
%(w_s,u_{\ell+s+1},\dots,u_m,w_s).
%\]
%One of these two sub-walks is the boundary walk of a face~$\psi_{2k}$, while the other is the boundary walk of a face~$\chi_{2k-1}$, and these faces are corresponding to the embedding of a splitting graph $U_1$ of $G$ resulting from $U_0=H$ by merging the path $P'_{2k-1}$ and $P''_{2k-1}$. The directions of $\psi_{2k}$ and $\chi_{2k-1}$ are inherited from the original orientation of $B_0$. Let us prune the histories of the nodes, by removing all edges labeled~$P'_{2k-1}$ and~$P''_{2k-1}$, and let us denote  the boundary walks extracted from $B_0$ that corresponds to the face~$\chi_{2k-1}$ of the planar embedding of~$U_1$ by~$B_1$. 
%
%By repeating the same construction on the boundary walk of~$B_1$, using the histories of the nodes related to edges labeled~$P'_{2k-2}$ and~$P''_{2k-2}$, the duplication of a path $P_{2k-2}$ can be identified. This path connects a face~$\psi_{2k-1}$ with a face~$\chi_{2k-2}$ of a planar embedding of a splitting graph $U_2$ of $G$ resulting from $U_1$ by merging the path $P'_{2k-2}$ and $P''_{2k-2}$.  
% 
%By iterating the construction $2k-1$ times, a planar embedding of a splitting graph $U_{2k-1}$ of $G$, containing $2k$ special faces $\psi_1,\dots,\psi_{2k}$,  whose boundaries are all directed clockwise, by inheriting from the original orientation of~$\phi^*$. At this stages, the histories of the nodes have edges labeled by labels in $\{C'_1,\dots ,C'_k,C''_1,\dots ,C''_k\}$. 
%
%By using the edges labeled $C'_k$ and $C''_k$ in the histories of the nodes, one can identify two faces $\phi'_k$ and $\phi''_k$ with respective boundary walks $v'_0, \dots, v'_r$ and $v''_0, \dots, v''_r$, where, for every $i=0,\dots,r$, the two nodes $v'_i$ and $v''_i$ are  resulting from splitting a same node into two. Moreover, walking along the boundary of one of thee face according to the clockwise direction results in visiting the vertices in index-order $0,1,\dots,r$, while walking along the boundary of the other face according to  the clockwise direction results in visiting the vertices in index-order $r,r-1,\dots,0$. By identifying $v'_i$ and $v''_i$ into a single node $v_i$ for every~$i$, the faces $\phi'_k$ and $\phi''_k$ are therefore glued together, decreasing by~2 the number of faces, and creating a handle. Merging the nodes  $v'_i$ and $v''_i$ into $v_i$ for every~$i$ results in a graph $U_{2k}$, which is a splitting of the graph~$G$. The planar embedding of $U_{2k-1}$ induces an embedding of $U_{2k}$ in~$\T_1$.  
%
%One can then prune the histories of the nodes by removing the edges labeled  $C'_k$ and $C''_k$, and repeat the process, for identifying the two faces $\phi'_{k-1}$ and $\phi''_{k-1}$. By iterating $k$~times this process, all pairs of faces $(\phi'_i,\phi''_i)$, $i=1,\dots,k$, are eliminated, and the resulting graph $U_{3k-1}$ is simply $G$, with an embedding in~$\T_k$  induced by the  embeddings of $U_{2k+i}$ in $\T_{i+1}$ for $i=1,\dots,k-1$. 
\end{proof}

Thanks to Theorem~\ref{theo:certif-Tk-centralized}, the outcome of this section is that 
\[
c=(H^*,f^*,\phi^*,B^*,\hist^*)
\]
is a certificate that $G$ can be embedded in~$\T_k$. This certificate~$c$ and its corresponding verification algorithm are  however centralized. In the next section, we show how to distribute both the certificate~$c$, and the verification protocol. 

%%%%%%% Old version of Eric %%%%%%%
%\eric{je commence ici}
%
%Conversely, let $G$ be a graph, and assume that we have an embedding $U_0$ of a graph of  $H$,  in $\T_0$, such that $H$ is a splitting of $G$, and  $U_0$ has a  special  face  $\phi^*$ such that: 
%\begin{itemize}
%\item  each  vertex  on the boundary of $\phi^*$ is a vertex obtained by splitting,  
%\item   each  vertex  on the boundary of $\phi^*$ is given a set of labels,   chosen in the set $$\{C'_1, C'_2,... , C'_{k},  C''_1, C''_2,... , C''_{k},  P'_1, P'_2, ... , P'_{2k-1},  P''_1, P''_2,... , P''_{2k-1}\}.$$ 
%\end{itemize}
%Assume that a walk direction, say ``clockwise",   of  the boundary of $\phi^*$ is fixed.\\
%
%Let $j$,  $0 \leq j \leq 2k-1$, be an integer. We say that \emph{the reconstruction process succeeds until level $j$}, if 
% a sequence $(U_{0}, U_{1}, ... U_{j})$ of (planar) embeddings can be constructed in such a way that,   
%for each $i$, $0 \leq i < j $,  $U_i$ satisfies the following conditions. 
%\begin{itemize}
%\item the vertices   labeled by $P'_{2k-1-i}$  form a path $(w'_0, w'_1, ...   ,w'_s)$ 
%the vertices   labeled by $P''_{2k-1-i}$  form a path $(w''_s, w''_{s-1}, ...  ,w''_0)$. These two paths are pairwise disjoint, of the same length,  a included in the boundary of a same face $\phi$, not linked by an edge of the boundary of  $\phi$, and  directed by the direction of boundary walk of  $\phi$.  
%\item     for each  $r$, $0 \leq r \leq s$, the vertices $w'_r$ and $w''_r$ are in the same splitting class,  and have the same labels, (other than  $P'_{2k-1-i}$ and $P''_{2k-1-i})$. 
% 
%\end{itemize}
%When this holds,   $U_{i+1}$ is obtained  from $ U_i$ by identifying the two paths above,(merging elements $w'_r$ and $w''_r$)  and  deleting the labels $P'_{2k-1-i}$ and $P''_{2k-1-i}$. By this way,  the face $\phi$ of $ U_i$ is  replaced by two faces $\psi$ and $\psi'$  of $U_{i+1}$. The boundaries of these to faces  are  directed, this direction is inherited from the direction of $\phi$.  Notice that the identification of paths preserves the planarity, and that the new graph is also a splitting of $G$ .  
%
%Assume that the reconstruction process succeeds until level $i$. An easy  induction shows   that,  for $0 \leq i \leq 2k-1$,
%$U_{i}$ is a planar 2-cell embedding of a splitting of $G$ with   $i+1$ special faces whose boundaries contain all vertices obtained by splitting, these boundaries being directed clockwise.  The only remaining labels  on $U_i$ are on the set $$\{C'_1, C'_2,... , C'_{k},  C''_1, C''_2,... , C''_{k},  P'_1, P'_2, ... , P'_{2k-1- i},  P''_1, P''_2,... , P''_{2k-1 -i}\}. $$  
%In particular, if the reconstruction process succeeds until level $2k-1$,  then, in $U_{2k-1}$, only cycle labels remain since all path labels have been previously deleted. On the other hand, $U_{2k-1}$ contains $2k$ special faces,  whose  boundaries are directed clockwise.   \\
%
%
%
%% a sequence $(U_{k}, U_{k+1}, ... U_{j})$ of embeddings can be constructed in such a way that,   
%%for each $i$, $2k-1 \leq i < j $,  $U_i$ satisfies the following conditions. 
%%\begin{itemize}
%%\item there exists a face $\phi'$ whose a boundary walk,  following the direction attributed to  the boundary,  is   $(v'_0, v'_1, ... , v'_p = v'_0)$, where   $\{v'_0, v'_1, ... , 
%%v'_{p- 1}\}$ is the set of vertices labeled by  $C'_{ 3k -1 -i }$, 
%%and  there exists 
%%a face $\phi''$ whose   a boundary walk following the direction attributed to  the boundary, is $(v''_p, v''_{p- 1},  ... , v''_0 = v''_p)$, where   $\{v''_0, v''_1, ... , v''_{p- 1}\}$ is the set of vertices labeled by  $C''_{ 3k -1 -i }$. 
%%These two boundary walks are disjoint,  of the same length.
%% \item     for each  $r$, $0 \leq r \leq p$, the vertices $v'_r$ and $v''_r$ are in the same splitting class. 
%%  %\item   if $ P = ( v'_t = w_0, w_1, ...,  w_s = v''_u)$ is a path linking $\phi'$ and $\phi''$,  then $v'_{t+1}$  and $v''_{u+1}$ are in opposites sides of $P$. 
%%   \end{itemize}
%%  
%  
%%  When this holds,   $U_{i+1}$ is obtained  from $ U_i$ by identifying the two boundary cycles above (merging $w'_r$ and $w''_r$)  and  deleting the labels $C'_{ 3k -1 -i }$ and $C''_{ 3k -1 -j }$. By this way,  the faces $\phi'$ and $\phi''$ of $ U_i$ are deleted, which makes that   $U_{i+1}$ has two faces less than $U_{i}$. 
%%  
%%  Assume that the reconstruction process succeeds until level $3k-1$. One can check, by induction,  that,  for $0 \leq i \leq 2k-1$,
%%$U_{i}$ is a planar 2-cell embedding on  $\T_{ i -2k+1}$ with   $6k -2 -2i$ special faces whose boundaries contain all vertices obtained by splitting, these boundaries being directed.   The only remaining labels  on $U_i$ are on the set $\{C'_1, C'_2,... , C'_{ 3k -1 -j },  C''_1, C''_2,... , C''_{ 3k -1 -j }, \}$    
%%
%% The only point to be checked carefully is the fact that,  when passing  from $U_{i}$ to $U_{i+1}$,  the orientability is preserved, i.e.   a handle (and not  a ``Klein bottle like'')  is used for constructing $U_{i+1}$ from $U_{i}$.  Hence the fact that  $U_{i}$ is an embedding $\T_{ i -2k+1}$  implies that $U_{i+1}$ is an embedding $\T_{ i -2k+2}$. This fact  is ensured by the use of inherited  boundary directions. 
%% 
%
%%\eric{A partir d'ci,  j'h'\'esite entre deux variantes}
%
%
%%\eric{Premi\`ere variante, qui suit la construction}
%
%Now let $j$,  $2k \leq j \leq 3k-1$, be an integer. We say that the \emph{reconstruction process succeeds until level $j$} if it succeeds until level $2k-1$ and,  moreover, 
% a sequence $(U_{k}, U_{k+1}, ... U_{j})$ of embeddings can be constructed in such a way that,   
%for each $i$, $2k-1 \leq i < j $,  $U_i$ satisfies the following conditions. 
%\begin{itemize}
%\item there exists a regular face $\phi'$ such that  $(v'_0, v'_1, ... , v'_p = v'_0)$ is  boundary walk of $\phi'$, following  the direction attributed to  the boundary, where   $\{v'_0, v'_1, ... , 
%v'_{p- 1}\}$ is the set of vertices labeled by  $C'_{ 3k -1 -i }$, 
%and  there exists 
%a face $\phi''$ whose   such that  $(v''_p, v''_{p- 1},  ... , v''_0 = v''_p)$ is a boundary walk following the direction attributed to  the boundary  of $\phi''$ ,
% where   $\{v''_0, v''_1, ... , v''_{p- 1}\}$ is the set of vertices labeled by  $C''_{ 3k -1 -i }$. 
%These two boundary walks are disjoint,  of the same length.
% \item     for each  $r$, $0 \leq r \leq p$, the vertices $v'_r$ and $v''_r$ are in the same splitting class, and have the same labels, (other than  $C'_{ 3k -1 -i }$ and $C''_{ 3k -1 -i })$. 
%  %\item   if $ P = ( v'_t = w_0, w_1, ...,  w_s = v''_u)$ is a path linking $\phi'$ and $\phi''$,  then $v'_{t+1}$  and $v''_{u+1}$ are in opposites sides of $P$. 
%   \end{itemize}
%  
%  
%  When this holds,   $U_{i+1}$ is obtained  from $ U_i$ by identifying the two boundary cycles above (merging $v'_r$ and $v''_r$)  and  deleting the labels $C'_{ 3k -1 -i }$ and $C''_{ 3k -1 -j }$. By this way,  the faces $\phi'$ and $\phi''$ of $ U_i$ are deleted, which makes that   $U_{i+1}$ has two faces less than $U_{i}$. 
%  
% Assume that the reconstruction process succeeds until level $i$, $2k-1 \leq i \leq 3k-1$. An induction shows that $U_{i}$ is a planar 2-cell embedding on  $\T_{ i -2k+1}$ with   $6k -2 -2i$ special faces whose boundaries contain all vertices obtained by splitting, these boundaries being directed.   The only remaining labels  on $U_i$ are on the set $\{C'_1, C'_2,... , C'_{ 3k -1 -j },  C''_1, C''_2,... , C''_{ 3k -1 -j }, \}$    
%
%The only point to be checked carefully is the fact that,  when passing  from $U_{i}$ to $U_{i+1}$,  the orientability is preserved, i.e.   a handle (and not  a ``Klein bottle like'')  is used for constructing $U_{i+1}$ from $U_{i}$.  Hence the fact that  $U_{i}$ is an embedding $\T_{ i -2k+1}$  implies that $U_{i+1}$ is an embedding $\T_{ i -2k+2}$. This fact  is ensured by the use of inherited  boundary directions : these directions are all clockwise in   $U_{i}$, which ensures  to create a handle by identify  boundaries of faces $\phi'$  and  $\phi''$. Thus,  $U_{i+1}$ is a embedding in an orientable surface and, using Lemma   \ref{euler}, this surface is $\T_{ i -2k+2}$. 
% 
% 
% \begin{lemma}
%If there exists an embedding  $U_0$ for which reconstruction  succeeds until level $3k-1$, 
%then the graph $G$ is of genus at most $k$. 
%\end{lemma}
%
%\begin{proof}
%if the hypothesis holds, then $U_{3k-1}$ is an embedding of graph $G'$, splitting of $G$,  on  $\T_{ 3k-1 -2k+1} = \T_k$  with $6k-2 -2(3k-1) = 0 $ special faces.  since there is no special face, there is no split vertex, thus $G' = G$, which gives the result. 
%\end{proof}
%
%
%
%
%%
%%\eric{Deuxi\`eme variante, simplificatrice}
%%
%%
%%
%%
%%
%%We say that \emph{the reconstruction process fully  succeeds}  if it succeeds until level $2k-1$ and,  moreover,  
%%\begin{itemize}
%%\item all special faces of $U_{2k-1}$ are regular, 
%%\item there exists a one-to-one mapping  $g$ from the set of special faces of $U_{2k-1}$ to the set  $\{C'_1, C'_2,... , C'_{k},  C''_1, C''_2,... , C''_{k} \}$ of cycle labels, such that  $g(\phi) = L $ if the set of  vertices of the boundary of $\phi$ is the set of vertices with the label $L$.  
%%\item let $i$,  $1 \leq 1 \leq k$, be an integer,  $(v'_0, v'_1, ... , v'_p = v'_0)$ be a clockwise boundary walk of the face $\phi'$  such that $ g(\phi')  = C'_i$ and $(v''_p, v''_{p- 1},  ... , v''_0 = v''_p)$ be a clockwise boundary walk of the face $\phi''$  such that $ g(\phi'')  = C''_i$. 
%%
%%These two boundary walks are disjoint,  of the same length, and for each  $r$, $0 \leq r \leq p$, the vertices $v'_r$ and $v''_r$ are in the same splitting class.
%%\end{itemize}
%%
%% 
%%
%%
%%\begin{lemma}
%%If there exists an embedding  $U_0$ for which reconstruction  fully succeeds, 
%%then the graph $G$ is of genus at most $k$. 
%%\end{lemma}
%%
%%\begin{proof}
%%
%%\end{proof}
%%
%\eric{je finis ici}
%%%%%%%



  

